The Transit Light Curve (TLC) Project. I. Four Consecutive Transits of the Exoplanet XO-1b

We present RIz photometry of four consecutive transits of the newly discovered exoplanet XO-1b. We improve upon the estimates of the transit parameters, finding the planetary radius to be R_P = 1.184 +0.028/-0.018 R_Jupiter and the stellar radius to be R_S = 0.928 +0.018/-0.013 R_Sun, assuming a stellar mass of M_S = 1.00 +/- 0.03 M_Sun. The uncertainties in the planetary and stellar radii are dominated by the uncertainty in the stellar mass. These uncertainties increase by a factor of 2-3 if a more conservative uncertainty of 0.10 M_Sun is assumed for the stellar mass. Our estimate of the planetary radius is smaller than that reported by McCullough et al. (2006) and yields a mean density that is comparable to that of TrES-1 and HD 189733b. The timings of the transits have an accuracy ranging from 0.2 to 2.5 minutes, and are marginally consistent with a uniform period.

==> tab1.tex <==
\begin{deluxetable}{lcccc}
\tabletypesize{\normalsize}
\tablecaption{Photometry of XO-1\label{tbl:photometry}}
\tablewidth{0pt}

\tablehead{
\colhead{Telescope} & \colhead{Filter} & \colhead{HJD} & \colhead{Relative flux} & \colhead{Uncertainty} \\
}

\startdata
         FLWO48 & $z$ & $2453883.70727$   &     $1.00125$   &        $0.00147$   \\
         FLWO48 & $z$ & $2453883.70776$   &     $0.99952$   &        $0.00148$   \\
         FLWO48 & $z$ & $2453883.70825$   &     $0.99668$   &        $0.00148$   \\
         FLWO48 & $z$ & $2453883.70874$   &     $1.00139$   &        $0.00147$   \\
         FLWO48 & $z$ & $2453883.70921$   &     $1.00184$   &        $0.00147$   \\
         FLWO48 & $z$ & $2453883.70970$   &     $1.00093$   &        $0.00147$   \\
         FLWO48 & $z$ & $2453883.71019$   &     $1.00156$   &        $0.00147$   \\
         FLWO48 & $z$ & $2453883.71067$   &     $1.00179$   &        $0.00147$   \\
         FLWO48 & $z$ & $2453883.71115$   &     $1.00037$   &        $0.00147$   \\
         FLWO48 & $z$ & $2453883.71165$   &     $0.99938$   &        $0.00148$   \\
         FLWO48 & $z$ & $2453883.71214$   &     $0.99752$   &        $0.00148$   \\
         FLWO48 & $z$ & $2453883.71262$   &     $1.00014$   &        $0.00147$   \\
         FLWO48 & $z$ & $2453883.71311$   &     $0.99799$   &        $0.00148$   \\
         FLWO48 & $z$ & $2453883.71359$   &     $0.99822$   &        $0.00147$   \\
         FLWO48 & $z$ & $2453883.71407$   &     $1.00000$   &        $0.00147$   \\
         FLWO48 & $z$ & $2453883.71457$   &     $1.00016$   &        $0.00147$   \\
         FLWO48 & $z$ & $2453883.71504$   &     $1.00009$   &        $0.00147$   \\
         FLWO48 & $z$ & $2453883.71553$   &     $1.00215$   &        $0.00147$   \\
         FLWO48 & $z$ & $2453883.71602$   &     $0.99820$   &        $0.00147$   \\
         FLWO48 & $z$ & $2453883.71650$   &     $0.99930$   &        $0.00147$   \\
         FLWO48 & $z$ & $2453883.71698$   &     $1.00211$   &        $0.00147$   \\
         FLWO48 & $z$ & $2453883.71747$   &     $1.00201$   &        $0.00147$   \\
         FLWO48 & $z$ & $2453883.71796$   &     $1.00334$   &        $0.00147$   \\
         FLWO48 & $z$ & $2453883.71843$   &     $0.99889$   &        $0.00147$   \\
         FLWO48 & $z$ & $2453883.71892$   &     $0.99798$   &        $0.00147$   \\
         FLWO48 & $z$ & $2453883.71940$   &     $0.99817$   &        $0.00147$   \\
         FLWO48 & $z$ & $2453883.71989$   &     $1.00044$   &        $0.00147$   \\
         FLWO48 & $z$ & $2453883.72036$   &     $1.00090$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.72083$   &     $1.00198$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.72130$   &     $1.00077$   &        $0.00147$   \\
         FLWO48 & $z$ & $2453883.72180$   &     $0.99832$   &        $0.00147$   \\
         FLWO48 & $z$ & $2453883.72229$   &     $1.00125$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.72277$   &     $0.99994$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.72327$   &     $0.99968$   &        $0.00147$   \\
         FLWO48 & $z$ & $2453883.72374$   &     $0.99878$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.72422$   &     $0.99700$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.72469$   &     $0.99786$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.72518$   &     $1.00155$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.72564$   &     $0.99915$   &        $0.00147$   \\
         FLWO48 & $z$ & $2453883.72613$   &     $1.00127$   &        $0.00147$   \\
         FLWO48 & $z$ & $2453883.72663$   &     $1.00339$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.72710$   &     $1.00322$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.72760$   &     $1.00086$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.72808$   &     $0.99870$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.72856$   &     $0.99552$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.72903$   &     $1.00208$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.72952$   &     $0.99908$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.73001$   &     $0.99796$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.73049$   &     $0.99742$   &        $0.00147$   \\
         FLWO48 & $z$ & $2453883.73099$   &     $0.99931$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.73146$   &     $0.99925$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.73196$   &     $1.00050$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.73245$   &     $0.99902$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.73294$   &     $1.00044$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.73342$   &     $1.00008$   &        $0.00147$   \\
         FLWO48 & $z$ & $2453883.73391$   &     $1.00259$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.73440$   &     $1.00239$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.73489$   &     $1.00106$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.73538$   &     $1.00200$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.73587$   &     $1.00070$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.73637$   &     $0.99548$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.73685$   &     $1.00220$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.73734$   &     $0.99966$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.73782$   &     $0.99827$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.73829$   &     $0.99895$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.73877$   &     $1.00032$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.73924$   &     $1.00167$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.73974$   &     $0.99893$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.74024$   &     $1.00040$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.74071$   &     $0.99830$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.74117$   &     $0.99981$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.74167$   &     $1.00134$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.74216$   &     $0.99910$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.74264$   &     $0.99971$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.74311$   &     $0.99950$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.74360$   &     $1.00037$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.74409$   &     $0.99961$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.74459$   &     $1.00222$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.74506$   &     $0.99872$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.74554$   &     $1.00109$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.74601$   &     $0.99959$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.74650$   &     $0.99836$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.74700$   &     $0.99870$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.74747$   &     $0.99761$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.74794$   &     $0.99828$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.74841$   &     $0.99564$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.74891$   &     $0.99474$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.74937$   &     $0.99385$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.74986$   &     $0.99488$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.75035$   &     $0.99481$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.75084$   &     $0.99354$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.75134$   &     $0.99402$   &        $0.00147$   \\
         FLWO48 & $z$ & $2453883.75181$   &     $0.99322$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.75227$   &     $0.99460$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.75277$   &     $0.99279$   &        $0.00147$   \\
         FLWO48 & $z$ & $2453883.75326$   &     $0.99112$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.75375$   &     $0.99240$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.75423$   &     $0.98971$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.75472$   &     $0.99146$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.75520$   &     $0.98634$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.75575$   &     $0.98948$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.75623$   &     $0.98759$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.75672$   &     $0.98695$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.75720$   &     $0.98449$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.75769$   &     $0.98663$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.75818$   &     $0.98236$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.75865$   &     $0.98404$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.75914$   &     $0.98722$   &        $0.00147$   \\
         FLWO48 & $z$ & $2453883.75964$   &     $0.98427$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.76011$   &     $0.98347$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.76059$   &     $0.98548$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.76108$   &     $0.98472$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.76157$   &     $0.98408$   &        $0.00147$   \\
         FLWO48 & $z$ & $2453883.76254$   &     $0.98255$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.76349$   &     $0.98049$   &        $0.00148$   \\
         FLWO48 & $z$ & $2453883.76398$   &     $0.98327$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.76445$   &     $0.98254$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.76491$   &     $0.98272$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.76541$   &     $0.98355$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.76587$   &     $0.98180$   &        $0.00147$   \\
         FLWO48 & $z$ & $2453883.76635$   &     $0.97985$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.76683$   &     $0.98433$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.76733$   &     $0.98276$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.76782$   &     $0.98241$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.76830$   &     $0.98348$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.76879$   &     $0.97960$   &        $0.00150$   \\
         FLWO48 & $z$ & $2453883.76926$   &     $0.98258$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.76975$   &     $0.98091$   &        $0.00147$   \\
         FLWO48 & $z$ & $2453883.77025$   &     $0.98165$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.77072$   &     $0.98296$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.77118$   &     $0.98299$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.77170$   &     $0.98254$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.77217$   &     $0.98156$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.77264$   &     $0.98064$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.77312$   &     $0.98087$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.77359$   &     $0.98190$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.77408$   &     $0.98214$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.77458$   &     $0.97930$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.77506$   &     $0.98182$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.77554$   &     $0.98045$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.77602$   &     $0.97938$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.77651$   &     $0.98230$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.77701$   &     $0.97995$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.77748$   &     $0.98265$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.77798$   &     $0.98066$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.77845$   &     $0.98149$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.77893$   &     $0.97920$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.77941$   &     $0.98015$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.77989$   &     $0.98031$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.78039$   &     $0.97949$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.78087$   &     $0.97894$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.78136$   &     $0.98056$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.78185$   &     $0.98178$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.78233$   &     $0.98091$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.78283$   &     $0.98041$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.78332$   &     $0.97924$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.78380$   &     $0.98210$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.78429$   &     $0.98238$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.78477$   &     $0.98088$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.78526$   &     $0.97982$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.78575$   &     $0.97968$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.78623$   &     $0.98084$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.78673$   &     $0.98123$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.78720$   &     $0.97877$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.78768$   &     $0.97898$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.78816$   &     $0.98018$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.78865$   &     $0.97953$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.78915$   &     $0.98071$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.78962$   &     $0.97953$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.79012$   &     $0.98058$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.79061$   &     $0.97961$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.79109$   &     $0.98181$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.79158$   &     $0.98049$   &        $0.00147$   \\
         FLWO48 & $z$ & $2453883.79208$   &     $0.97966$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.79255$   &     $0.97850$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.79304$   &     $0.97834$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.79353$   &     $0.98017$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.79401$   &     $0.98064$   &        $0.00142$   \\
         FLWO48 & $z$ & $2453883.79451$   &     $0.98081$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.79499$   &     $0.98050$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.79547$   &     $0.97992$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.79595$   &     $0.98030$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.79644$   &     $0.98053$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.79694$   &     $0.97977$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.79742$   &     $0.98180$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.79790$   &     $0.97997$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.79837$   &     $0.98156$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.79886$   &     $0.97783$   &        $0.00147$   \\
         FLWO48 & $z$ & $2453883.79935$   &     $0.97958$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.79983$   &     $0.97745$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.80033$   &     $0.98160$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.80079$   &     $0.98116$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.80129$   &     $0.98023$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.80178$   &     $0.98094$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.80225$   &     $0.97956$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.80272$   &     $0.98003$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.80321$   &     $0.98011$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.80370$   &     $0.97777$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.80424$   &     $0.98020$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.80472$   &     $0.98025$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.80520$   &     $0.97899$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.80567$   &     $0.98021$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.80616$   &     $0.97804$   &        $0.00147$   \\
         FLWO48 & $z$ & $2453883.80666$   &     $0.98067$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.80714$   &     $0.97978$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.80763$   &     $0.97835$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.80813$   &     $0.97966$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.80860$   &     $0.98094$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.80908$   &     $0.97952$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.80956$   &     $0.98228$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.81004$   &     $0.98027$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.81053$   &     $0.97844$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.81101$   &     $0.98081$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.81149$   &     $0.97845$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.81196$   &     $0.98109$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.81244$   &     $0.98163$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.81292$   &     $0.97824$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.81342$   &     $0.98204$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.81389$   &     $0.98105$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.81439$   &     $0.98210$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.81488$   &     $0.97895$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.81535$   &     $0.97997$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.81583$   &     $0.97864$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.81631$   &     $0.98028$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.81680$   &     $0.97940$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.81727$   &     $0.98017$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.81776$   &     $0.98023$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.81822$   &     $0.98076$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.81871$   &     $0.98087$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.81921$   &     $0.98126$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.82017$   &     $0.98227$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.82065$   &     $0.97967$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.82114$   &     $0.98024$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.82162$   &     $0.97955$   &        $0.00147$   \\
         FLWO48 & $z$ & $2453883.82212$   &     $0.98010$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.82259$   &     $0.98014$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.82309$   &     $0.97926$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.82356$   &     $0.97933$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.82404$   &     $0.97940$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.82454$   &     $0.98018$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.82502$   &     $0.98066$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.82553$   &     $0.97965$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.82600$   &     $0.98087$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.82647$   &     $0.97844$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.82697$   &     $0.97858$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.82746$   &     $0.98037$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.82794$   &     $0.97966$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.82844$   &     $0.97779$   &        $0.00147$   \\
         FLWO48 & $z$ & $2453883.82894$   &     $0.98126$   &        $0.00148$   \\
         FLWO48 & $z$ & $2453883.82944$   &     $0.98061$   &        $0.00147$   \\
         FLWO48 & $z$ & $2453883.82991$   &     $0.98221$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.83039$   &     $0.97926$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.83087$   &     $0.98013$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.83137$   &     $0.98019$   &        $0.00147$   \\
         FLWO48 & $z$ & $2453883.83185$   &     $0.98372$   &        $0.00147$   \\
         FLWO48 & $z$ & $2453883.83234$   &     $0.98022$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.83283$   &     $0.98103$   &        $0.00147$   \\
         FLWO48 & $z$ & $2453883.83333$   &     $0.97975$   &        $0.00147$   \\
         FLWO48 & $z$ & $2453883.83380$   &     $0.98112$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.83429$   &     $0.98218$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.83477$   &     $0.98311$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.83526$   &     $0.98132$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.83574$   &     $0.97995$   &        $0.00148$   \\
         FLWO48 & $z$ & $2453883.83623$   &     $0.98119$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.83669$   &     $0.98136$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.83718$   &     $0.98355$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.83767$   &     $0.98101$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.83815$   &     $0.98118$   &        $0.00147$   \\
         FLWO48 & $z$ & $2453883.83863$   &     $0.97683$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.83911$   &     $0.98072$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.83960$   &     $0.98313$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.84010$   &     $0.98144$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.84059$   &     $0.98017$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.84106$   &     $0.97990$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.84154$   &     $0.98272$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.84203$   &     $0.97963$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.84253$   &     $0.98161$   &        $0.00147$   \\
         FLWO48 & $z$ & $2453883.84300$   &     $0.98157$   &        $0.00147$   \\
         FLWO48 & $z$ & $2453883.84349$   &     $0.98006$   &        $0.00147$   \\
         FLWO48 & $z$ & $2453883.84399$   &     $0.98243$   &        $0.00147$   \\
         FLWO48 & $z$ & $2453883.84446$   &     $0.98349$   &        $0.00147$   \\
         FLWO48 & $z$ & $2453883.84496$   &     $0.97736$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.84543$   &     $0.98436$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.84591$   &     $0.98363$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.84639$   &     $0.98180$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.84689$   &     $0.98265$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.84739$   &     $0.98042$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.84786$   &     $0.98477$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.84836$   &     $0.98125$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.84885$   &     $0.98452$   &        $0.00147$   \\
         FLWO48 & $z$ & $2453883.84931$   &     $0.98352$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.84982$   &     $0.98177$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.85029$   &     $0.98074$   &        $0.00147$   \\
         FLWO48 & $z$ & $2453883.85079$   &     $0.98703$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.85127$   &     $0.98214$   &        $0.00147$   \\
         FLWO48 & $z$ & $2453883.85176$   &     $0.98413$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.85225$   &     $0.98517$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.85278$   &     $0.98495$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.85327$   &     $0.98526$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.85375$   &     $0.98700$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.85425$   &     $0.98962$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.85474$   &     $0.98753$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.85521$   &     $0.98758$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.85571$   &     $0.98804$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.85620$   &     $0.98945$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.85668$   &     $0.99137$   &        $0.00144$   \\
         FLWO48 & $z$ & $2453883.85717$   &     $0.98890$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.85764$   &     $0.98907$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.85815$   &     $0.99150$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.85863$   &     $0.98986$   &        $0.00147$   \\
         FLWO48 & $z$ & $2453883.85910$   &     $0.99788$   &        $0.00148$   \\
         FLWO48 & $z$ & $2453883.85956$   &     $0.99021$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.86005$   &     $0.99130$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.86052$   &     $0.99417$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.86101$   &     $0.99502$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.86151$   &     $0.99433$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.86199$   &     $0.99623$   &        $0.00147$   \\
         FLWO48 & $z$ & $2453883.86248$   &     $0.99767$   &        $0.00147$   \\
         FLWO48 & $z$ & $2453883.86295$   &     $0.99743$   &        $0.00148$   \\
         FLWO48 & $z$ & $2453883.86343$   &     $0.99716$   &        $0.00147$   \\
         FLWO48 & $z$ & $2453883.86392$   &     $0.99699$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.86440$   &     $0.99728$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.86489$   &     $1.00076$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.86536$   &     $1.00028$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.86584$   &     $1.00045$   &        $0.00147$   \\
         FLWO48 & $z$ & $2453883.86632$   &     $0.99968$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.86681$   &     $0.99937$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.86729$   &     $0.99799$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.86778$   &     $1.00462$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.86827$   &     $1.00124$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.86876$   &     $1.00056$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.86926$   &     $0.99654$   &        $0.00147$   \\
         FLWO48 & $z$ & $2453883.86974$   &     $0.99912$   &        $0.00147$   \\
         FLWO48 & $z$ & $2453883.87021$   &     $1.00056$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.87070$   &     $0.99992$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.87118$   &     $1.00086$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.87168$   &     $1.00028$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.87217$   &     $0.99740$   &        $0.00148$   \\
         FLWO48 & $z$ & $2453883.87267$   &     $0.99764$   &        $0.00147$   \\
         FLWO48 & $z$ & $2453883.87313$   &     $1.00118$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.87361$   &     $1.00178$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.87411$   &     $1.00128$   &        $0.00147$   \\
         FLWO48 & $z$ & $2453883.87460$   &     $0.99939$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.87508$   &     $0.99990$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.87557$   &     $1.00107$   &        $0.00147$   \\
         FLWO48 & $z$ & $2453883.87606$   &     $1.00112$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.87653$   &     $1.00034$   &        $0.00147$   \\
         FLWO48 & $z$ & $2453883.87712$   &     $1.00000$   &        $0.00147$   \\
         FLWO48 & $z$ & $2453883.87762$   &     $0.99785$   &        $0.00145$   \\
         FLWO48 & $z$ & $2453883.87809$   &     $0.99972$   &        $0.00147$   \\
         FLWO48 & $z$ & $2453883.87858$   &     $0.99844$   &        $0.00147$   \\
         FLWO48 & $z$ & $2453883.87908$   &     $1.00077$   &        $0.00147$   \\
         FLWO48 & $z$ & $2453883.87956$   &     $0.99900$   &        $0.00147$   \\
         FLWO48 & $z$ & $2453883.88005$   &     $0.99968$   &        $0.00147$   \\
         FLWO48 & $z$ & $2453883.88054$   &     $0.99920$   &        $0.00147$   \\
         FLWO48 & $z$ & $2453883.88102$   &     $0.99894$   &        $0.00148$   \\
         FLWO48 & $z$ & $2453883.88148$   &     $0.99941$   &        $0.00148$   \\
         FLWO48 & $z$ & $2453883.88198$   &     $0.99971$   &        $0.00147$   \\
         FLWO48 & $z$ & $2453883.88247$   &     $0.99853$   &        $0.00148$   \\
         FLWO48 & $z$ & $2453883.88295$   &     $1.00289$   &        $0.00148$   \\
         FLWO48 & $z$ & $2453883.88344$   &     $1.00270$   &        $0.00147$   \\
         FLWO48 & $z$ & $2453883.88393$   &     $1.00167$   &        $0.00147$   \\
         FLWO48 & $z$ & $2453883.88444$   &     $0.99946$   &        $0.00148$   \\
         FLWO48 & $z$ & $2453883.88490$   &     $1.00220$   &        $0.00147$   \\
         FLWO48 & $z$ & $2453883.88539$   &     $1.00035$   &        $0.00148$   \\
         FLWO48 & $z$ & $2453883.88587$   &     $0.99955$   &        $0.00147$   \\
         FLWO48 & $z$ & $2453883.88636$   &     $0.99814$   &        $0.00147$   \\
         FLWO48 & $z$ & $2453883.88684$   &     $1.00015$   &        $0.00147$   \\
         FLWO48 & $z$ & $2453883.88733$   &     $0.99878$   &        $0.00147$   \\
         FLWO48 & $z$ & $2453883.88780$   &     $0.99967$   &        $0.00147$   \\
         FLWO48 & $z$ & $2453883.88828$   &     $1.00100$   &        $0.00147$   \\
         FLWO48 & $z$ & $2453883.88876$   &     $0.99876$   &        $0.00148$   \\
         FLWO48 & $z$ & $2453883.88924$   &     $1.00012$   &        $0.00148$   \\
         FLWO48 & $z$ & $2453883.88975$   &     $1.00168$   &        $0.00147$   \\
         FLWO48 & $z$ & $2453883.89022$   &     $0.99975$   &        $0.00147$   \\
         FLWO48 & $z$ & $2453883.89068$   &     $0.99755$   &        $0.00147$   \\
         FLWO48 & $z$ & $2453883.89118$   &     $0.99860$   &        $0.00148$   \\
         FLWO48 & $z$ & $2453883.89165$   &     $0.99875$   &        $0.00148$   \\
         FLWO48 & $z$ & $2453883.89213$   &     $0.99850$   &        $0.00148$   \\
         FLWO48 & $z$ & $2453883.89263$   &     $0.99844$   &        $0.00148$   \\
         FLWO48 & $z$ & $2453883.89313$   &     $1.00175$   &        $0.00150$   \\
         FLWO48 & $z$ & $2453883.89360$   &     $1.00195$   &        $0.00148$   \\
         FLWO48 & $z$ & $2453883.89409$   &     $1.00105$   &        $0.00148$   \\
         FLWO48 & $z$ & $2453883.89457$   &     $1.00087$   &        $0.00148$   \\
         FLWO48 & $z$ & $2453883.89506$   &     $0.99871$   &        $0.00148$   \\
         FLWO48 & $z$ & $2453883.89554$   &     $0.99988$   &        $0.00148$   \\
         FLWO48 & $z$ & $2453883.89603$   &     $0.99961$   &        $0.00148$   \\
         FLWO48 & $z$ & $2453883.89651$   &     $1.00062$   &        $0.00148$   \\
         FLWO48 & $z$ & $2453883.89698$   &     $1.00001$   &        $0.00148$   \\
         FLWO48 & $z$ & $2453883.89747$   &     $1.00031$   &        $0.00148$   \\
         FLWO48 & $z$ & $2453883.89797$   &     $0.99822$   &        $0.00150$   \\
         FLWO48 & $z$ & $2453883.89844$   &     $1.00167$   &        $0.00148$   \\
         FLWO48 & $z$ & $2453883.89891$   &     $0.99773$   &        $0.00148$   \\
         FLWO48 & $z$ & $2453883.89941$   &     $1.00241$   &        $0.00148$   \\
         FLWO48 & $z$ & $2453883.89990$   &     $0.99939$   &        $0.00150$   \\
         FLWO48 & $z$ & $2453883.90040$   &     $0.99933$   &        $0.00148$   \\
         FLWO48 & $z$ & $2453883.90088$   &     $1.00048$   &        $0.00150$   \\
         FLWO48 & $z$ & $2453883.90138$   &     $1.00206$   &        $0.00150$   \\
         FLWO48 & $z$ & $2453883.90185$   &     $0.99912$   &        $0.00150$   \\
         FLWO48 & $z$ & $2453883.90235$   &     $1.00035$   &        $0.00150$   \\
         FLWO48 & $z$ & $2453883.90284$   &     $1.00213$   &        $0.00150$   \\
         FLWO48 & $z$ & $2453883.90334$   &     $0.99845$   &        $0.00150$   \\
         FLWO48 & $z$ & $2453883.90382$   &     $1.00022$   &        $0.00150$   \\
         FLWO48 & $z$ & $2453883.90432$   &     $1.00036$   &        $0.00150$   \\
         FLWO48 & $z$ & $2453883.90481$   &     $1.00070$   &        $0.00150$   \\
         FLWO48 & $z$ & $2453883.90529$   &     $1.00136$   &        $0.00150$   \\
         FLWO48 & $z$ & $2453883.90578$   &     $0.99908$   &        $0.00150$   \\
         FLWO48 & $z$ & $2453883.90627$   &     $0.99932$   &        $0.00150$   \\
         FLWO48 & $z$ & $2453883.90677$   &     $1.00225$   &        $0.00150$   \\
         FLWO48 & $z$ & $2453883.90725$   &     $0.99838$   &        $0.00151$   \\
         FLWO48 & $z$ & $2453883.90772$   &     $1.00202$   &        $0.00151$   \\
         FLWO48 & $z$ & $2453883.90821$   &     $0.99765$   &        $0.00151$   \\
         FLWO48 & $z$ & $2453883.90869$   &     $1.00129$   &        $0.00151$   \\
         FLWO48 & $z$ & $2453883.90918$   &     $0.99996$   &        $0.00151$   \\
         FLWO48 & $z$ & $2453883.90966$   &     $0.99963$   &        $0.00151$   \\
         FLWO48 & $z$ & $2453883.91012$   &     $0.99976$   &        $0.00151$   \\
         FLWO48 & $z$ & $2453887.65708$   &     $1.00118$   &        $0.00130$   \\
         FLWO48 & $z$ & $2453887.65819$   &     $1.00179$   &        $0.00130$   \\
         FLWO48 & $z$ & $2453887.65902$   &     $0.99898$   &        $0.00130$   \\
         FLWO48 & $z$ & $2453887.65950$   &     $1.00035$   &        $0.00130$   \\
         FLWO48 & $z$ & $2453887.65999$   &     $0.99945$   &        $0.00129$   \\
         FLWO48 & $z$ & $2453887.66046$   &     $1.00008$   &        $0.00129$   \\
         FLWO48 & $z$ & $2453887.66093$   &     $0.99967$   &        $0.00129$   \\
         FLWO48 & $z$ & $2453887.66141$   &     $0.99991$   &        $0.00129$   \\
         FLWO48 & $z$ & $2453887.66190$   &     $0.99903$   &        $0.00129$   \\
         FLWO48 & $z$ & $2453887.66238$   &     $0.99973$   &        $0.00129$   \\
         FLWO48 & $z$ & $2453887.66288$   &     $1.00032$   &        $0.00129$   \\
         FLWO48 & $z$ & $2453887.66336$   &     $0.99958$   &        $0.00127$   \\
         FLWO48 & $z$ & $2453887.66384$   &     $1.00110$   &        $0.00127$   \\
         FLWO48 & $z$ & $2453887.66449$   &     $0.99901$   &        $0.00127$   \\
         FLWO48 & $z$ & $2453887.66541$   &     $1.00121$   &        $0.00127$   \\
         FLWO48 & $z$ & $2453887.66589$   &     $1.00168$   &        $0.00127$   \\
         FLWO48 & $z$ & $2453887.66637$   &     $1.00080$   &        $0.00126$   \\
         FLWO48 & $z$ & $2453887.66687$   &     $1.00106$   &        $0.00126$   \\
         FLWO48 & $z$ & $2453887.66737$   &     $0.99921$   &        $0.00126$   \\
         FLWO48 & $z$ & $2453887.66784$   &     $0.99908$   &        $0.00126$   \\
         FLWO48 & $z$ & $2453887.66833$   &     $0.99969$   &        $0.00126$   \\
         FLWO48 & $z$ & $2453887.66879$   &     $1.00011$   &        $0.00126$   \\
         FLWO48 & $z$ & $2453887.66928$   &     $0.99994$   &        $0.00126$   \\
         FLWO48 & $z$ & $2453887.66977$   &     $1.00012$   &        $0.00126$   \\
         FLWO48 & $z$ & $2453887.67026$   &     $0.99900$   &        $0.00126$   \\
         FLWO48 & $z$ & $2453887.67075$   &     $1.00075$   &        $0.00126$   \\
         FLWO48 & $z$ & $2453887.67123$   &     $0.99951$   &        $0.00126$   \\
         FLWO48 & $z$ & $2453887.67172$   &     $0.99942$   &        $0.00126$   \\
         FLWO48 & $z$ & $2453887.67221$   &     $0.99948$   &        $0.00126$   \\
         FLWO48 & $z$ & $2453887.67268$   &     $1.00312$   &        $0.00126$   \\
         FLWO48 & $z$ & $2453887.67315$   &     $1.00182$   &        $0.00126$   \\
         FLWO48 & $z$ & $2453887.67363$   &     $0.99889$   &        $0.00126$   \\
         FLWO48 & $z$ & $2453887.67411$   &     $0.99712$   &        $0.00126$   \\
         FLWO48 & $z$ & $2453887.67460$   &     $0.99932$   &        $0.00126$   \\
         FLWO48 & $z$ & $2453887.67509$   &     $0.99894$   &        $0.00126$   \\
         FLWO48 & $z$ & $2453887.67556$   &     $0.99859$   &        $0.00126$   \\
         FLWO48 & $z$ & $2453887.67604$   &     $1.00092$   &        $0.00126$   \\
         FLWO48 & $z$ & $2453887.67651$   &     $1.00072$   &        $0.00125$   \\
         FLWO48 & $z$ & $2453887.67700$   &     $0.99924$   &        $0.00126$   \\
         FLWO48 & $z$ & $2453887.67748$   &     $1.00273$   &        $0.00125$   \\
         FLWO48 & $z$ & $2453887.67845$   &     $1.00033$   &        $0.00125$   \\
         FLWO48 & $z$ & $2453887.67894$   &     $1.00006$   &        $0.00126$   \\
         FLWO48 & $z$ & $2453887.67945$   &     $0.99871$   &        $0.00125$   \\
         FLWO48 & $z$ & $2453887.67992$   &     $0.99784$   &        $0.00125$   \\
         FLWO48 & $z$ & $2453887.68041$   &     $1.00230$   &        $0.00125$   \\
         FLWO48 & $z$ & $2453887.68090$   &     $0.99931$   &        $0.00125$   \\
         FLWO48 & $z$ & $2453887.68138$   &     $0.99824$   &        $0.00125$   \\
         FLWO48 & $z$ & $2453887.68189$   &     $1.00039$   &        $0.00125$   \\
         FLWO48 & $z$ & $2453887.68238$   &     $0.99789$   &        $0.00125$   \\
         FLWO48 & $z$ & $2453887.68286$   &     $1.00009$   &        $0.00125$   \\
         FLWO48 & $z$ & $2453887.68335$   &     $0.99914$   &        $0.00125$   \\
         FLWO48 & $z$ & $2453887.68383$   &     $0.99857$   &        $0.00125$   \\
         FLWO48 & $z$ & $2453887.68430$   &     $1.00028$   &        $0.00125$   \\
         FLWO48 & $z$ & $2453887.68482$   &     $0.99772$   &        $0.00125$   \\
         FLWO48 & $z$ & $2453887.68528$   &     $0.99945$   &        $0.00125$   \\
         FLWO48 & $z$ & $2453887.68576$   &     $0.99962$   &        $0.00125$   \\
         FLWO48 & $z$ & $2453887.68624$   &     $0.99970$   &        $0.00125$   \\
         FLWO48 & $z$ & $2453887.68672$   &     $1.00121$   &        $0.00124$   \\
         FLWO48 & $z$ & $2453887.68720$   &     $0.99922$   &        $0.00124$   \\
         FLWO48 & $z$ & $2453887.68769$   &     $0.99914$   &        $0.00124$   \\
         FLWO48 & $z$ & $2453887.68817$   &     $0.99822$   &        $0.00124$   \\
         FLWO48 & $z$ & $2453887.68866$   &     $0.99735$   &        $0.00124$   \\
         FLWO48 & $z$ & $2453887.68915$   &     $0.99583$   &        $0.00124$   \\
         FLWO48 & $z$ & $2453887.68970$   &     $0.99556$   &        $0.00124$   \\
         FLWO48 & $z$ & $2453887.69020$   &     $0.99629$   &        $0.00124$   \\
         FLWO48 & $z$ & $2453887.69067$   &     $0.99540$   &        $0.00124$   \\
         FLWO48 & $z$ & $2453887.69116$   &     $0.99306$   &        $0.00124$   \\
         FLWO48 & $z$ & $2453887.69165$   &     $0.99470$   &        $0.00124$   \\
         FLWO48 & $z$ & $2453887.69212$   &     $0.99246$   &        $0.00124$   \\
         FLWO48 & $z$ & $2453887.69261$   &     $0.99112$   &        $0.00124$   \\
         FLWO48 & $z$ & $2453887.69308$   &     $0.99293$   &        $0.00124$   \\
         FLWO48 & $z$ & $2453887.69356$   &     $0.99311$   &        $0.00124$   \\
         FLWO48 & $z$ & $2453887.69404$   &     $0.99030$   &        $0.00124$   \\
         FLWO48 & $z$ & $2453887.69454$   &     $0.99006$   &        $0.00124$   \\
         FLWO48 & $z$ & $2453887.69502$   &     $0.99104$   &        $0.00124$   \\
         FLWO48 & $z$ & $2453887.69550$   &     $0.98752$   &        $0.00124$   \\
         FLWO48 & $z$ & $2453887.69599$   &     $0.98700$   &        $0.00124$   \\
         FLWO48 & $z$ & $2453887.69649$   &     $0.98916$   &        $0.00124$   \\
         FLWO48 & $z$ & $2453887.69696$   &     $0.98605$   &        $0.00124$   \\
         FLWO48 & $z$ & $2453887.69745$   &     $0.98475$   &        $0.00124$   \\
         FLWO48 & $z$ & $2453887.69793$   &     $0.98809$   &        $0.00124$   \\
         FLWO48 & $z$ & $2453887.69843$   &     $0.98218$   &        $0.00124$   \\
         FLWO48 & $z$ & $2453887.69892$   &     $0.98595$   &        $0.00124$   \\
         FLWO48 & $z$ & $2453887.69939$   &     $0.98454$   &        $0.00124$   \\
         FLWO48 & $z$ & $2453887.69988$   &     $0.98428$   &        $0.00124$   \\
         FLWO48 & $z$ & $2453887.70035$   &     $0.98568$   &        $0.00124$   \\
         FLWO48 & $z$ & $2453887.70084$   &     $0.98346$   &        $0.00124$   \\
         FLWO48 & $z$ & $2453887.70131$   &     $0.98416$   &        $0.00124$   \\
         FLWO48 & $z$ & $2453887.70180$   &     $0.98429$   &        $0.00124$   \\
         FLWO48 & $z$ & $2453887.70227$   &     $0.98302$   &        $0.00124$   \\
         FLWO48 & $z$ & $2453887.70276$   &     $0.98225$   &        $0.00124$   \\
         FLWO48 & $z$ & $2453887.70323$   &     $0.98285$   &        $0.00124$   \\
         FLWO48 & $z$ & $2453887.70372$   &     $0.98432$   &        $0.00124$   \\
         FLWO48 & $z$ & $2453887.70418$   &     $0.98070$   &        $0.00124$   \\
         FLWO48 & $z$ & $2453887.70466$   &     $0.98216$   &        $0.00124$   \\
         FLWO48 & $z$ & $2453887.70516$   &     $0.98312$   &        $0.00124$   \\
         FLWO48 & $z$ & $2453887.70564$   &     $0.98280$   &        $0.00124$   \\
         FLWO48 & $z$ & $2453887.70612$   &     $0.98194$   &        $0.00124$   \\
         FLWO48 & $z$ & $2453887.70660$   &     $0.98378$   &        $0.00124$   \\
         FLWO48 & $z$ & $2453887.70709$   &     $0.98231$   &        $0.00124$   \\
         FLWO48 & $z$ & $2453887.70757$   &     $0.98194$   &        $0.00123$   \\
         FLWO48 & $z$ & $2453887.70807$   &     $0.98186$   &        $0.00124$   \\
         FLWO48 & $z$ & $2453887.70855$   &     $0.98192$   &        $0.00123$   \\
         FLWO48 & $z$ & $2453887.70902$   &     $0.98110$   &        $0.00123$   \\
         FLWO48 & $z$ & $2453887.70950$   &     $0.98213$   &        $0.00123$   \\
         FLWO48 & $z$ & $2453887.70997$   &     $0.98017$   &        $0.00124$   \\
         FLWO48 & $z$ & $2453887.71046$   &     $0.97991$   &        $0.00124$   \\
         FLWO48 & $z$ & $2453887.71094$   &     $0.98388$   &        $0.00124$   \\
         FLWO48 & $z$ & $2453887.71143$   &     $0.98067$   &        $0.00124$   \\
         FLWO48 & $z$ & $2453887.71190$   &     $0.98007$   &        $0.00124$   \\
         FLWO48 & $z$ & $2453887.71238$   &     $0.97879$   &        $0.00124$   \\
         FLWO48 & $z$ & $2453887.71286$   &     $0.98170$   &        $0.00123$   \\
         FLWO48 & $z$ & $2453887.71334$   &     $0.98011$   &        $0.00124$   \\
         FLWO48 & $z$ & $2453887.71404$   &     $0.98589$   &        $0.00123$   \\
         FLWO48 & $z$ & $2453887.71469$   &     $0.97996$   &        $0.00123$   \\
         FLWO48 & $z$ & $2453887.71517$   &     $0.98242$   &        $0.00123$   \\
         FLWO48 & $z$ & $2453887.71564$   &     $0.98035$   &        $0.00123$   \\
         FLWO48 & $z$ & $2453887.71612$   &     $0.98147$   &        $0.00123$   \\
         FLWO48 & $z$ & $2453887.71659$   &     $0.98091$   &        $0.00123$   \\
         FLWO48 & $z$ & $2453887.71709$   &     $0.98165$   &        $0.00123$   \\
         FLWO48 & $z$ & $2453887.71755$   &     $0.98147$   &        $0.00123$   \\
         FLWO48 & $z$ & $2453887.71804$   &     $0.98196$   &        $0.00123$   \\
         FLWO48 & $z$ & $2453887.71852$   &     $0.97916$   &        $0.00123$   \\
         FLWO48 & $z$ & $2453887.71901$   &     $0.98079$   &        $0.00123$   \\
         FLWO48 & $z$ & $2453887.71948$   &     $0.97866$   &        $0.00123$   \\
         FLWO48 & $z$ & $2453887.71996$   &     $0.98023$   &        $0.00123$   \\
         FLWO48 & $z$ & $2453887.72044$   &     $0.97829$   &        $0.00122$   \\
         FLWO48 & $z$ & $2453887.72092$   &     $0.97957$   &        $0.00123$   \\
         FLWO48 & $z$ & $2453887.72140$   &     $0.98139$   &        $0.00122$   \\
         FLWO48 & $z$ & $2453887.72189$   &     $0.98203$   &        $0.00122$   \\
         FLWO48 & $z$ & $2453887.72237$   &     $0.97750$   &        $0.00122$   \\
         FLWO48 & $z$ & $2453887.72285$   &     $0.97947$   &        $0.00122$   \\
         FLWO48 & $z$ & $2453887.72335$   &     $0.98257$   &        $0.00123$   \\
         FLWO48 & $z$ & $2453887.72384$   &     $0.98066$   &        $0.00122$   \\
         FLWO48 & $z$ & $2453887.72432$   &     $0.98064$   &        $0.00122$   \\
         FLWO48 & $z$ & $2453887.72480$   &     $0.97887$   &        $0.00122$   \\
         FLWO48 & $z$ & $2453887.72529$   &     $0.97992$   &        $0.00122$   \\
         FLWO48 & $z$ & $2453887.72576$   &     $0.97935$   &        $0.00122$   \\
         FLWO48 & $z$ & $2453887.72624$   &     $0.97973$   &        $0.00122$   \\
         FLWO48 & $z$ & $2453887.72673$   &     $0.98147$   &        $0.00122$   \\
         FLWO48 & $z$ & $2453887.72720$   &     $0.98124$   &        $0.00122$   \\
         FLWO48 & $z$ & $2453887.72769$   &     $0.98068$   &        $0.00122$   \\
         FLWO48 & $z$ & $2453887.72819$   &     $0.98045$   &        $0.00122$   \\
         FLWO48 & $z$ & $2453887.72866$   &     $0.97812$   &        $0.00122$   \\
         FLWO48 & $z$ & $2453887.72914$   &     $0.97995$   &        $0.00122$   \\
         FLWO48 & $z$ & $2453887.72961$   &     $0.98054$   &        $0.00122$   \\
         FLWO48 & $z$ & $2453887.73008$   &     $0.97952$   &        $0.00122$   \\
         FLWO48 & $z$ & $2453887.73057$   &     $0.98350$   &        $0.00122$   \\
         FLWO48 & $z$ & $2453887.73105$   &     $0.97737$   &        $0.00122$   \\
         FLWO48 & $z$ & $2453887.73152$   &     $0.98302$   &        $0.00120$   \\
         FLWO48 & $z$ & $2453887.73201$   &     $0.98186$   &        $0.00120$   \\
         FLWO48 & $z$ & $2453887.73249$   &     $0.98200$   &        $0.00120$   \\
         FLWO48 & $z$ & $2453887.73299$   &     $0.97775$   &        $0.00122$   \\
         FLWO48 & $z$ & $2453887.73348$   &     $0.97999$   &        $0.00122$   \\
         FLWO48 & $z$ & $2453887.73395$   &     $0.98020$   &        $0.00120$   \\
         FLWO48 & $z$ & $2453887.73443$   &     $0.97960$   &        $0.00120$   \\
         FLWO48 & $z$ & $2453887.73490$   &     $0.97846$   &        $0.00120$   \\
         FLWO48 & $z$ & $2453887.73538$   &     $0.97946$   &        $0.00120$   \\
         FLWO48 & $z$ & $2453887.73586$   &     $0.97947$   &        $0.00120$   \\
         FLWO48 & $z$ & $2453887.73635$   &     $0.98021$   &        $0.00120$   \\
         FLWO48 & $z$ & $2453887.73682$   &     $0.97939$   &        $0.00120$   \\
         FLWO48 & $z$ & $2453887.73731$   &     $0.98281$   &        $0.00120$   \\
         FLWO48 & $z$ & $2453887.73778$   &     $0.97866$   &        $0.00120$   \\
         FLWO48 & $z$ & $2453887.73828$   &     $0.97969$   &        $0.00120$   \\
         FLWO48 & $z$ & $2453887.73877$   &     $0.98116$   &        $0.00120$   \\
         FLWO48 & $z$ & $2453887.73926$   &     $0.98083$   &        $0.00120$   \\
         FLWO48 & $z$ & $2453887.73973$   &     $0.98090$   &        $0.00120$   \\
         FLWO48 & $z$ & $2453887.74022$   &     $0.97906$   &        $0.00120$   \\
         FLWO48 & $z$ & $2453887.74071$   &     $0.98066$   &        $0.00120$   \\
         FLWO48 & $z$ & $2453887.74121$   &     $0.97954$   &        $0.00120$   \\
         FLWO48 & $z$ & $2453887.74169$   &     $0.98089$   &        $0.00120$   \\
         FLWO48 & $z$ & $2453887.74217$   &     $0.97875$   &        $0.00120$   \\
         FLWO48 & $z$ & $2453887.74266$   &     $0.98053$   &        $0.00120$   \\
         FLWO48 & $z$ & $2453887.74314$   &     $0.97695$   &        $0.00120$   \\
         FLWO48 & $z$ & $2453887.74362$   &     $0.97951$   &        $0.00120$   \\
         FLWO48 & $z$ & $2453887.74410$   &     $0.98099$   &        $0.00120$   \\
         FLWO48 & $z$ & $2453887.74459$   &     $0.98053$   &        $0.00120$   \\
         FLWO48 & $z$ & $2453887.74507$   &     $0.97995$   &        $0.00120$   \\
         FLWO48 & $z$ & $2453887.74557$   &     $0.98123$   &        $0.00120$   \\
         FLWO48 & $z$ & $2453887.74606$   &     $0.97928$   &        $0.00120$   \\
         FLWO48 & $z$ & $2453887.74653$   &     $0.97850$   &        $0.00120$   \\
         FLWO48 & $z$ & $2453887.74700$   &     $0.98055$   &        $0.00120$   \\
         FLWO48 & $z$ & $2453887.74748$   &     $0.97948$   &        $0.00120$   \\
         FLWO48 & $z$ & $2453887.74798$   &     $0.98004$   &        $0.00120$   \\
         FLWO48 & $z$ & $2453887.74845$   &     $0.98106$   &        $0.00120$   \\
         FLWO48 & $z$ & $2453887.74894$   &     $0.98089$   &        $0.00120$   \\
         FLWO48 & $z$ & $2453887.74941$   &     $0.97698$   &        $0.00120$   \\
         FLWO48 & $z$ & $2453887.74989$   &     $0.97875$   &        $0.00120$   \\
         FLWO48 & $z$ & $2453887.75039$   &     $0.98080$   &        $0.00120$   \\
         FLWO48 & $z$ & $2453887.75086$   &     $0.98037$   &        $0.00120$   \\
         FLWO48 & $z$ & $2453887.75135$   &     $0.97931$   &        $0.00120$   \\
         FLWO48 & $z$ & $2453887.75183$   &     $0.97941$   &        $0.00120$   \\
         FLWO48 & $z$ & $2453887.75231$   &     $0.98149$   &        $0.00120$   \\
         FLWO48 & $z$ & $2453887.75281$   &     $0.97913$   &        $0.00120$   \\
         FLWO48 & $z$ & $2453887.75329$   &     $0.97795$   &        $0.00120$   \\
         FLWO48 & $z$ & $2453887.75377$   &     $0.97972$   &        $0.00120$   \\
         FLWO48 & $z$ & $2453887.75424$   &     $0.98260$   &        $0.00120$   \\
         FLWO48 & $z$ & $2453887.75471$   &     $0.98203$   &        $0.00120$   \\
         FLWO48 & $z$ & $2453887.75521$   &     $0.98220$   &        $0.00120$   \\
         FLWO48 & $z$ & $2453887.75569$   &     $0.97852$   &        $0.00120$   \\
         FLWO48 & $z$ & $2453887.75618$   &     $0.97994$   &        $0.00120$   \\
         FLWO48 & $z$ & $2453887.75667$   &     $0.98069$   &        $0.00120$   \\
         FLWO48 & $z$ & $2453887.75715$   &     $0.98074$   &        $0.00120$   \\
         FLWO48 & $z$ & $2453887.75762$   &     $0.97809$   &        $0.00120$   \\
         FLWO48 & $z$ & $2453887.75812$   &     $0.98023$   &        $0.00120$   \\
         FLWO48 & $z$ & $2453887.75860$   &     $0.97875$   &        $0.00120$   \\
         FLWO48 & $z$ & $2453887.75908$   &     $0.98033$   &        $0.00120$   \\
         FLWO48 & $z$ & $2453887.75956$   &     $0.97984$   &        $0.00120$   \\
         FLWO48 & $z$ & $2453887.76005$   &     $0.98002$   &        $0.00120$   \\
         FLWO48 & $z$ & $2453887.76054$   &     $0.98036$   &        $0.00120$   \\
         FLWO48 & $z$ & $2453887.76103$   &     $0.98052$   &        $0.00120$   \\
         FLWO48 & $z$ & $2453887.76151$   &     $0.98132$   &        $0.00120$   \\
         FLWO48 & $z$ & $2453887.76197$   &     $0.97831$   &        $0.00120$   \\
         FLWO48 & $z$ & $2453887.76246$   &     $0.97793$   &        $0.00120$   \\
         FLWO48 & $z$ & $2453887.76308$   &     $0.98148$   &        $0.00120$   \\
         FLWO48 & $z$ & $2453887.76357$   &     $0.97806$   &        $0.00120$   \\
         FLWO48 & $z$ & $2453887.76407$   &     $0.97983$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.76455$   &     $0.98188$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.76502$   &     $0.97951$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.76551$   &     $0.98056$   &        $0.00120$   \\
         FLWO48 & $z$ & $2453887.76600$   &     $0.98134$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.76649$   &     $0.98021$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.76695$   &     $0.98113$   &        $0.00120$   \\
         FLWO48 & $z$ & $2453887.76743$   &     $0.97973$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.76791$   &     $0.98035$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.76838$   &     $0.98273$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.76886$   &     $0.98091$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.76933$   &     $0.97950$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.76981$   &     $0.98213$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.77029$   &     $0.97980$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.77078$   &     $0.98074$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.77128$   &     $0.97921$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.77175$   &     $0.98067$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.77224$   &     $0.98007$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.77274$   &     $0.98098$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.77321$   &     $0.98060$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.77368$   &     $0.98031$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.77416$   &     $0.98089$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.77465$   &     $0.98292$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.77511$   &     $0.98106$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.77559$   &     $0.98198$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.77609$   &     $0.98106$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.77657$   &     $0.98138$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.77704$   &     $0.98124$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.77752$   &     $0.98067$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.77800$   &     $0.98200$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.77848$   &     $0.98241$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.77897$   &     $0.98211$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.77946$   &     $0.98063$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.77993$   &     $0.97890$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.78040$   &     $0.98130$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.78088$   &     $0.98205$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.78138$   &     $0.98120$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.78186$   &     $0.97997$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.78234$   &     $0.98162$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.78284$   &     $0.98144$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.78330$   &     $0.98125$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.78379$   &     $0.98094$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.78426$   &     $0.98227$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.78474$   &     $0.98124$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.78521$   &     $0.98171$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.78569$   &     $0.98088$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.78618$   &     $0.98207$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.78666$   &     $0.98266$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.78733$   &     $0.98029$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.78783$   &     $0.98184$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.78830$   &     $0.98331$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.78880$   &     $0.98187$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.78928$   &     $0.98320$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.78975$   &     $0.98390$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.79024$   &     $0.98165$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.79071$   &     $0.98335$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.79120$   &     $0.98433$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.79168$   &     $0.98419$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.79217$   &     $0.98173$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.79265$   &     $0.98283$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.79314$   &     $0.98516$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.79363$   &     $0.98491$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.79411$   &     $0.98364$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.79459$   &     $0.98286$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.79508$   &     $0.98484$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.79556$   &     $0.98441$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.79602$   &     $0.98647$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.79651$   &     $0.98526$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.79698$   &     $0.98635$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.79747$   &     $0.98824$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.79795$   &     $0.98792$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.79843$   &     $0.98876$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.79893$   &     $0.99128$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.79940$   &     $0.99273$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.79990$   &     $0.99186$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.80039$   &     $0.99326$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.80085$   &     $0.99384$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.80135$   &     $0.99370$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.80181$   &     $0.99543$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.80229$   &     $0.99357$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.80279$   &     $0.99486$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.80328$   &     $0.99401$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.80375$   &     $0.99556$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.80425$   &     $0.99827$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.80473$   &     $0.99726$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.80522$   &     $0.99672$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.80570$   &     $0.99868$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.80620$   &     $0.99914$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.80668$   &     $0.99825$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.80716$   &     $0.99979$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.80763$   &     $0.99964$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.80810$   &     $0.99686$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.80859$   &     $0.99794$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.80907$   &     $1.00170$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.80955$   &     $1.00102$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.81005$   &     $0.99918$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.81055$   &     $1.00172$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.81102$   &     $0.99949$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.81153$   &     $1.00091$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.81202$   &     $0.99851$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.81250$   &     $0.99951$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.81299$   &     $1.00072$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.81349$   &     $1.00104$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.81397$   &     $0.99994$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.81446$   &     $0.99922$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.81493$   &     $0.99805$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.81541$   &     $0.99805$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.81589$   &     $0.99849$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.81639$   &     $1.00046$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.81685$   &     $0.99954$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.81735$   &     $0.99875$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.81784$   &     $0.99980$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.81831$   &     $0.99900$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.81879$   &     $1.00181$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.81929$   &     $0.99935$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.81977$   &     $1.00048$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.82026$   &     $0.99929$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.82076$   &     $1.00202$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.82122$   &     $0.99907$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.82172$   &     $0.99959$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.82220$   &     $0.99870$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.82268$   &     $0.99913$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.82315$   &     $0.99913$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.82363$   &     $1.00068$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.82412$   &     $1.00014$   &        $0.00120$   \\
         FLWO48 & $z$ & $2453887.82460$   &     $0.99934$   &        $0.00120$   \\
         FLWO48 & $z$ & $2453887.82511$   &     $0.99710$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.82558$   &     $0.99940$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.82606$   &     $1.00000$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.82654$   &     $1.00077$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.82703$   &     $0.99917$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.82750$   &     $1.00170$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.82799$   &     $0.99973$   &        $0.00120$   \\
         FLWO48 & $z$ & $2453887.82847$   &     $1.00145$   &        $0.00119$   \\
         FLWO48 & $z$ & $2453887.82896$   &     $0.99837$   &        $0.00120$   \\
         FLWO48 & $z$ & $2453887.82944$   &     $1.00084$   &        $0.00120$   \\
         FLWO48 & $z$ & $2453887.82992$   &     $1.00090$   &        $0.00120$   \\
         FLWO48 & $z$ & $2453887.83038$   &     $1.00090$   &        $0.00120$   \\
         FLWO48 & $z$ & $2453887.83087$   &     $1.00012$   &        $0.00120$   \\
         FLWO48 & $z$ & $2453887.83137$   &     $0.99866$   &        $0.00120$   \\
         FLWO48 & $z$ & $2453887.83184$   &     $0.99889$   &        $0.00120$   \\
         FLWO48 & $z$ & $2453887.83232$   &     $1.00057$   &        $0.00120$   \\
         FLWO48 & $z$ & $2453887.83279$   &     $1.00091$   &        $0.00120$   \\
         FLWO48 & $z$ & $2453887.83328$   &     $0.99972$   &        $0.00120$   \\
         FLWO48 & $z$ & $2453887.83375$   &     $0.99874$   &        $0.00120$   \\
         FLWO48 & $z$ & $2453887.83423$   &     $1.00263$   &        $0.00120$   \\
         FLWO48 & $z$ & $2453887.83471$   &     $1.00080$   &        $0.00120$   \\
         FLWO48 & $z$ & $2453887.83521$   &     $1.00207$   &        $0.00120$   \\
         FLWO48 & $z$ & $2453887.83629$   &     $0.99874$   &        $0.00120$   \\
         FLWO48 & $z$ & $2453887.83676$   &     $1.00000$   &        $0.00120$   \\
         FLWO48 & $z$ & $2453887.83724$   &     $0.99763$   &        $0.00120$   \\
         FLWO48 & $z$ & $2453887.83771$   &     $1.00058$   &        $0.00120$   \\
         FLWO48 & $z$ & $2453887.83820$   &     $0.99923$   &        $0.00120$   \\
         FLWO48 & $z$ & $2453887.83868$   &     $0.99826$   &        $0.00120$   \\
         FLWO48 & $z$ & $2453887.83919$   &     $1.00030$   &        $0.00120$   \\
         FLWO48 & $z$ & $2453887.83965$   &     $1.00129$   &        $0.00120$   \\
         FLWO48 & $z$ & $2453887.84014$   &     $1.00008$   &        $0.00120$   \\
         FLWO48 & $z$ & $2453887.84064$   &     $0.99953$   &        $0.00120$   \\
         FLWO48 & $z$ & $2453887.84112$   &     $1.00197$   &        $0.00120$   \\
         FLWO48 & $z$ & $2453887.84161$   &     $0.99937$   &        $0.00120$   \\
         FLWO48 & $z$ & $2453887.84209$   &     $1.00035$   &        $0.00120$   \\
         FLWO48 & $z$ & $2453887.84256$   &     $1.00021$   &        $0.00120$   \\
         FLWO48 & $z$ & $2453887.84305$   &     $0.99930$   &        $0.00122$   \\
         FLWO48 & $z$ & $2453887.84351$   &     $1.00019$   &        $0.00120$   \\
         FLWO48 & $z$ & $2453887.84399$   &     $0.99846$   &        $0.00122$   \\
         FLWO48 & $z$ & $2453887.84447$   &     $1.00017$   &        $0.00120$   \\
         FLWO48 & $z$ & $2453887.84493$   &     $1.00065$   &        $0.00122$   \\
         FLWO48 & $z$ & $2453887.84543$   &     $1.00108$   &        $0.00120$   \\
         FLWO48 & $z$ & $2453887.84592$   &     $0.99920$   &        $0.00120$   \\
         FLWO48 & $z$ & $2453887.84638$   &     $0.99993$   &        $0.00122$   \\
         FLWO48 & $z$ & $2453887.84687$   &     $0.99951$   &        $0.00120$   \\
         FLWO48 & $z$ & $2453887.84737$   &     $1.00160$   &        $0.00120$   \\
         FLWO48 & $z$ & $2453887.84785$   &     $0.99874$   &        $0.00122$   \\
         FLWO48 & $z$ & $2453887.84835$   &     $1.00060$   &        $0.00122$   \\
         FLWO48 & $z$ & $2453887.84883$   &     $1.00011$   &        $0.00122$   \\
         FLWO48 & $z$ & $2453887.84932$   &     $0.99967$   &        $0.00122$   \\
         FLWO48 & $z$ & $2453887.84980$   &     $1.00033$   &        $0.00122$   \\
         FLWO48 & $z$ & $2453887.85028$   &     $0.99877$   &        $0.00122$   \\
         FLWO48 & $z$ & $2453887.85078$   &     $1.00132$   &        $0.00120$   \\
         FLWO48 & $z$ & $2453887.85126$   &     $0.99985$   &        $0.00122$   \\
         FLWO48 & $z$ & $2453887.85175$   &     $1.00039$   &        $0.00122$   \\
         FLWO48 & $z$ & $2453887.85224$   &     $1.00006$   &        $0.00122$   \\
         FLWO48 & $z$ & $2453887.85272$   &     $1.00005$   &        $0.00122$   \\
         FLWO48 & $z$ & $2453887.85322$   &     $1.00253$   &        $0.00122$   \\
         FLWO48 & $z$ & $2453887.85368$   &     $0.99928$   &        $0.00122$   \\
         FLWO48 & $z$ & $2453887.85416$   &     $0.99943$   &        $0.00122$   \\
         FLWO48 & $z$ & $2453887.85465$   &     $1.00158$   &        $0.00122$   \\
         FLWO48 & $z$ & $2453887.85514$   &     $1.00003$   &        $0.00122$   \\
         FLWO48 & $z$ & $2453887.85564$   &     $1.00125$   &        $0.00122$   \\
      Palomar60 & $R$ & $2453875.77023$   &     $1.00144$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.77094$   &     $1.00290$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.77165$   &     $1.00074$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.77242$   &     $1.00088$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.77315$   &     $1.00095$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.77390$   &     $0.99715$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.77462$   &     $1.00108$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.77540$   &     $1.00338$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.77615$   &     $1.00171$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.77691$   &     $1.00174$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.77765$   &     $1.00155$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.77838$   &     $1.00025$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.77914$   &     $1.00045$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.77988$   &     $1.00111$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.78063$   &     $1.00148$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.78142$   &     $1.00032$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.78216$   &     $1.00251$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.78298$   &     $1.00004$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.78373$   &     $1.00235$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.78446$   &     $1.00039$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.78519$   &     $0.99777$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.78593$   &     $1.00108$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.79713$   &     $1.00155$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.79791$   &     $1.00090$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.79869$   &     $1.00189$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.79948$   &     $1.00118$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.80028$   &     $0.99971$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.80105$   &     $1.00100$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.80185$   &     $1.00240$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.80262$   &     $1.00205$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.80341$   &     $1.00046$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.80421$   &     $0.99873$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.80502$   &     $0.99908$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.80583$   &     $0.99936$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.80668$   &     $0.99850$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.80746$   &     $0.99918$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.80828$   &     $0.99808$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.80907$   &     $0.99880$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.80987$   &     $1.00005$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.81067$   &     $0.99983$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.81147$   &     $1.00106$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.81224$   &     $0.99963$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.81304$   &     $0.99972$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.81387$   &     $0.99729$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.81470$   &     $1.00019$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.81553$   &     $0.99876$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.81632$   &     $0.99872$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.81714$   &     $0.99842$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.81796$   &     $1.00043$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.81876$   &     $1.00162$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.81961$   &     $0.99966$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.82040$   &     $0.99895$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.82119$   &     $1.00129$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.82202$   &     $0.99880$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.82291$   &     $0.99690$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.82373$   &     $1.00136$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.82458$   &     $1.00068$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.82540$   &     $0.99954$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.82623$   &     $0.99858$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.82702$   &     $0.99791$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.82782$   &     $1.00065$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.82870$   &     $1.00182$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.82951$   &     $1.00181$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.83036$   &     $1.00116$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.83120$   &     $0.99778$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.83206$   &     $1.00084$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.83297$   &     $1.00128$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.83378$   &     $0.99985$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.83465$   &     $0.99881$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.83555$   &     $0.99977$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.83638$   &     $1.00028$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.83722$   &     $0.99732$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.83809$   &     $0.99946$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.83898$   &     $0.99951$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.83980$   &     $0.99537$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.84063$   &     $0.99627$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.84153$   &     $0.99585$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.84241$   &     $0.99738$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.84329$   &     $1.00123$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.84417$   &     $0.99965$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.84501$   &     $0.99744$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.84584$   &     $0.99951$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.84671$   &     $0.99739$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.84760$   &     $0.99730$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.84843$   &     $0.99720$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.84927$   &     $0.99791$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.85047$   &     $0.99889$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.85136$   &     $1.00000$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.85222$   &     $0.99603$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.85310$   &     $0.99966$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.85400$   &     $0.99904$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.85487$   &     $1.00189$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.85572$   &     $0.99756$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.85662$   &     $0.99730$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.85751$   &     $1.00105$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.85841$   &     $1.00131$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.85931$   &     $0.99662$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.86021$   &     $0.99896$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.86112$   &     $1.00010$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.86204$   &     $0.99883$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.86295$   &     $0.99970$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.86385$   &     $0.99711$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.86470$   &     $0.99790$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.86559$   &     $0.99618$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.86650$   &     $0.99555$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.86738$   &     $0.99459$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.86825$   &     $0.99378$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.86918$   &     $0.99463$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.87005$   &     $0.99054$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.87099$   &     $0.98808$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.87188$   &     $0.98924$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.87279$   &     $0.98738$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.87374$   &     $0.98379$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.87464$   &     $0.98556$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.87555$   &     $0.98451$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.87649$   &     $0.98334$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.87738$   &     $0.98283$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.87836$   &     $0.98701$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.87925$   &     $0.98496$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.88018$   &     $0.98065$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.88403$   &     $0.98253$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.88493$   &     $0.98500$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.88589$   &     $0.98354$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.88686$   &     $0.97547$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.88786$   &     $0.98120$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.88877$   &     $0.98208$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.88966$   &     $0.97966$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.89062$   &     $0.98143$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.89151$   &     $0.98002$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.89247$   &     $0.98093$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.89341$   &     $0.98112$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.89432$   &     $0.97949$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.89525$   &     $0.98334$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.89615$   &     $0.98021$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.89715$   &     $0.97755$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.89812$   &     $0.98084$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.89907$   &     $0.97871$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.90007$   &     $0.97919$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.90104$   &     $0.98046$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.90201$   &     $0.97463$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.90307$   &     $0.97578$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.90403$   &     $0.97528$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.90505$   &     $0.98288$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.90601$   &     $0.97942$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.90698$   &     $0.98058$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.90798$   &     $0.98062$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.90896$   &     $0.98218$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.91001$   &     $0.98128$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.91095$   &     $0.97811$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.91197$   &     $0.98044$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.91299$   &     $0.98008$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.91394$   &     $0.97822$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.91493$   &     $0.97964$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.91590$   &     $0.97705$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.91687$   &     $0.97660$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.91786$   &     $0.97992$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.93126$   &     $0.98419$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.93226$   &     $0.98201$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.93328$   &     $0.98012$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.93429$   &     $0.98109$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.93535$   &     $0.98430$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.93645$   &     $0.98037$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.93744$   &     $0.97921$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.93849$   &     $0.97596$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.93995$   &     $0.98343$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.94101$   &     $0.97865$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.94209$   &     $0.97889$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.94309$   &     $0.97886$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.94414$   &     $0.97784$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.94524$   &     $0.97876$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.94631$   &     $0.97888$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.94735$   &     $0.97908$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.94837$   &     $0.98056$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.94942$   &     $0.97873$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.95049$   &     $0.98023$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.95151$   &     $0.97951$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.95254$   &     $0.98086$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.95364$   &     $0.97921$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.95465$   &     $0.98289$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.95570$   &     $0.98070$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.95676$   &     $0.98168$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.95778$   &     $0.98208$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.95889$   &     $0.98091$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.95992$   &     $0.97668$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.96106$   &     $0.98175$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.96208$   &     $0.98308$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.96314$   &     $0.97717$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.96423$   &     $0.98501$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.96531$   &     $0.98451$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.96637$   &     $0.98315$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.96749$   &     $0.98330$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.96857$   &     $0.98248$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.96966$   &     $0.97951$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.97075$   &     $0.98410$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.97181$   &     $0.98924$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.97288$   &     $0.98365$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.97397$   &     $0.98458$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.97503$   &     $0.99160$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.97609$   &     $0.99182$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.97718$   &     $1.00298$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.97826$   &     $0.99682$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.97932$   &     $0.99141$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.98039$   &     $0.99701$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.98145$   &     $0.99438$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.98252$   &     $0.99334$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.98360$   &     $0.99852$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.98472$   &     $0.99501$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.98581$   &     $1.00032$   &        $0.00215$   \\
      Palomar60 & $R$ & $2453875.98691$   &     $0.99909$   &        $0.00215$   \\
         TopHAT & $I$ & $2453875.64414$   &     $1.00889$   &        $0.00386$   \\
         TopHAT & $I$ & $2453875.64668$   &     $0.99801$   &        $0.00368$   \\
         TopHAT & $I$ & $2453875.64922$   &     $1.00132$   &        $0.00386$   \\
         TopHAT & $I$ & $2453875.65176$   &     $1.00798$   &        $0.00386$   \\
         TopHAT & $I$ & $2453875.65429$   &     $1.00640$   &        $0.00381$   \\
         TopHAT & $I$ & $2453875.65684$   &     $1.00586$   &        $0.00331$   \\
         TopHAT & $I$ & $2453875.65937$   &     $1.00086$   &        $0.00326$   \\
         TopHAT & $I$ & $2453875.66190$   &     $0.99957$   &        $0.00322$   \\
         TopHAT & $I$ & $2453875.66449$   &     $0.99820$   &        $0.00326$   \\
         TopHAT & $I$ & $2453875.66704$   &     $1.00384$   &        $0.00322$   \\
         TopHAT & $I$ & $2453875.66958$   &     $0.99881$   &        $0.00294$   \\
         TopHAT & $I$ & $2453875.67213$   &     $0.99921$   &        $0.00299$   \\
         TopHAT & $I$ & $2453875.68705$   &     $1.00154$   &        $0.00381$   \\
         TopHAT & $I$ & $2453875.68958$   &     $0.99965$   &        $0.00331$   \\
         TopHAT & $I$ & $2453875.69217$   &     $0.99821$   &        $0.00285$   \\
         TopHAT & $I$ & $2453875.69470$   &     $1.00096$   &        $0.00285$   \\
         TopHAT & $I$ & $2453875.69724$   &     $1.00357$   &        $0.00289$   \\
         TopHAT & $I$ & $2453875.69978$   &     $1.00643$   &        $0.00303$   \\
         TopHAT & $I$ & $2453875.70236$   &     $1.00487$   &        $0.00253$   \\
         TopHAT & $I$ & $2453875.70491$   &     $1.00615$   &        $0.00345$   \\
         TopHAT & $I$ & $2453875.70744$   &     $1.00317$   &        $0.00308$   \\
         TopHAT & $I$ & $2453875.71004$   &     $1.00424$   &        $0.00248$   \\
         TopHAT & $I$ & $2453875.71263$   &     $0.99907$   &        $0.00322$   \\
         TopHAT & $I$ & $2453875.71774$   &     $1.00297$   &        $0.00308$   \\
         TopHAT & $I$ & $2453875.72283$   &     $1.00143$   &        $0.00289$   \\
         TopHAT & $I$ & $2453875.73044$   &     $1.00323$   &        $0.00266$   \\
         TopHAT & $I$ & $2453875.73304$   &     $0.99656$   &        $0.00331$   \\
         TopHAT & $I$ & $2453875.73558$   &     $1.00042$   &        $0.00266$   \\
         TopHAT & $I$ & $2453875.73855$   &     $1.00177$   &        $0.00262$   \\
         TopHAT & $I$ & $2453875.74108$   &     $0.99757$   &        $0.00271$   \\
         TopHAT & $I$ & $2453875.74362$   &     $0.99901$   &        $0.00271$   \\
         TopHAT & $I$ & $2453875.74615$   &     $1.00142$   &        $0.00253$   \\
         TopHAT & $I$ & $2453875.74869$   &     $1.00109$   &        $0.00289$   \\
         TopHAT & $I$ & $2453875.75123$   &     $0.99833$   &        $0.00253$   \\
         TopHAT & $I$ & $2453875.75377$   &     $1.00115$   &        $0.00266$   \\
         TopHAT & $I$ & $2453875.75632$   &     $1.00182$   &        $0.00289$   \\
         TopHAT & $I$ & $2453875.75884$   &     $0.99899$   &        $0.00257$   \\
         TopHAT & $I$ & $2453875.76139$   &     $1.00093$   &        $0.00244$   \\
         TopHAT & $I$ & $2453875.76393$   &     $0.99877$   &        $0.00262$   \\
         TopHAT & $I$ & $2453875.76647$   &     $0.99880$   &        $0.00285$   \\
         TopHAT & $I$ & $2453875.76900$   &     $1.00248$   &        $0.00276$   \\
         TopHAT & $I$ & $2453875.77155$   &     $1.00217$   &        $0.00294$   \\
         TopHAT & $I$ & $2453875.77408$   &     $1.01002$   &        $0.00731$   \\
         TopHAT & $I$ & $2453875.77661$   &     $1.00171$   &        $0.00285$   \\
         TopHAT & $I$ & $2453875.77914$   &     $0.99785$   &        $0.00248$   \\
         TopHAT & $I$ & $2453875.78169$   &     $0.99509$   &        $0.00262$   \\
         TopHAT & $I$ & $2453875.78423$   &     $0.99839$   &        $0.00230$   \\
         TopHAT & $I$ & $2453875.78676$   &     $0.99673$   &        $0.00239$   \\
         TopHAT & $I$ & $2453875.79227$   &     $1.00001$   &        $0.00230$   \\
         TopHAT & $I$ & $2453875.79481$   &     $0.99796$   &        $0.00271$   \\
         TopHAT & $I$ & $2453875.79734$   &     $0.99713$   &        $0.00262$   \\
         TopHAT & $I$ & $2453875.79988$   &     $0.99787$   &        $0.00271$   \\
         TopHAT & $I$ & $2453875.80241$   &     $0.99940$   &        $0.00198$   \\
         TopHAT & $I$ & $2453875.80495$   &     $0.99839$   &        $0.00235$   \\
         TopHAT & $I$ & $2453875.80749$   &     $0.99996$   &        $0.00257$   \\
         TopHAT & $I$ & $2453875.81008$   &     $0.99761$   &        $0.00262$   \\
         TopHAT & $I$ & $2453875.81262$   &     $1.00491$   &        $0.00285$   \\
         TopHAT & $I$ & $2453875.81770$   &     $1.00022$   &        $0.00212$   \\
         TopHAT & $I$ & $2453875.82278$   &     $1.00147$   &        $0.00207$   \\
         TopHAT & $I$ & $2453875.82537$   &     $1.00132$   &        $0.00244$   \\
         TopHAT & $I$ & $2453875.82792$   &     $1.00377$   &        $0.00239$   \\
         TopHAT & $I$ & $2453875.83045$   &     $1.00139$   &        $0.00253$   \\
         TopHAT & $I$ & $2453875.83300$   &     $0.99899$   &        $0.00235$   \\
         TopHAT & $I$ & $2453875.83554$   &     $0.99887$   &        $0.00235$   \\
         TopHAT & $I$ & $2453875.83812$   &     $1.00473$   &        $0.00225$   \\
         TopHAT & $I$ & $2453875.84364$   &     $1.00228$   &        $0.00230$   \\
         TopHAT & $I$ & $2453875.84871$   &     $1.00191$   &        $0.00239$   \\
         TopHAT & $I$ & $2453875.85125$   &     $1.00048$   &        $0.00221$   \\
         TopHAT & $I$ & $2453875.85380$   &     $1.00386$   &        $0.00257$   \\
         TopHAT & $I$ & $2453875.85887$   &     $1.00117$   &        $0.00189$   \\
         TopHAT & $I$ & $2453875.86143$   &     $1.00106$   &        $0.00207$   \\
         TopHAT & $I$ & $2453875.86397$   &     $0.99832$   &        $0.00230$   \\
         TopHAT & $I$ & $2453875.86650$   &     $0.99723$   &        $0.00216$   \\
         TopHAT & $I$ & $2453875.86905$   &     $0.99075$   &        $0.00202$   \\
         TopHAT & $I$ & $2453875.87159$   &     $0.99044$   &        $0.00239$   \\
         TopHAT & $I$ & $2453875.87412$   &     $0.98801$   &        $0.00230$   \\
         TopHAT & $I$ & $2453875.87667$   &     $0.98268$   &        $0.00289$   \\
         TopHAT & $I$ & $2453875.87920$   &     $0.98759$   &        $0.00216$   \\
         TopHAT & $I$ & $2453875.88175$   &     $0.98383$   &        $0.00235$   \\
         TopHAT & $I$ & $2453875.89776$   &     $0.97711$   &        $0.00193$   \\
         TopHAT & $I$ & $2453875.90034$   &     $0.98082$   &        $0.00253$   \\
         TopHAT & $I$ & $2453875.90288$   &     $0.98125$   &        $0.00216$   \\
         TopHAT & $I$ & $2453875.90542$   &     $0.98116$   &        $0.00212$   \\
         TopHAT & $I$ & $2453875.90801$   &     $0.98128$   &        $0.00253$   \\
         TopHAT & $I$ & $2453875.91060$   &     $0.98169$   &        $0.00221$   \\
         TopHAT & $I$ & $2453875.91320$   &     $0.98103$   &        $0.00225$   \\
         TopHAT & $I$ & $2453875.91574$   &     $0.98181$   &        $0.00257$   \\
         TopHAT & $I$ & $2453875.91834$   &     $0.98253$   &        $0.00257$   \\
         TopHAT & $I$ & $2453875.92092$   &     $0.97887$   &        $0.00266$   \\
         TopHAT & $I$ & $2453875.92352$   &     $0.97857$   &        $0.00198$   \\
         TopHAT & $I$ & $2453875.92605$   &     $0.97885$   &        $0.00257$   \\
         TopHAT & $I$ & $2453875.92864$   &     $0.97772$   &        $0.00230$   \\
         TopHAT & $I$ & $2453875.93119$   &     $0.97705$   &        $0.00248$   \\
         TopHAT & $I$ & $2453875.93372$   &     $0.97716$   &        $0.00221$   \\
         TopHAT & $I$ & $2453875.93633$   &     $0.97942$   &        $0.00212$   \\
         TopHAT & $I$ & $2453875.93887$   &     $0.97903$   &        $0.00294$   \\
         TopHAT & $I$ & $2453875.94146$   &     $0.98160$   &        $0.00244$   \\
         TopHAT & $I$ & $2453875.94400$   &     $0.97926$   &        $0.00257$   \\
         TopHAT & $I$ & $2453875.94703$   &     $0.97716$   &        $0.00244$   \\
         TopHAT & $I$ & $2453875.94961$   &     $0.97871$   &        $0.00212$   \\
         TopHAT & $I$ & $2453875.95215$   &     $0.97625$   &        $0.00239$   \\
         TopHAT & $I$ & $2453875.95469$   &     $0.98181$   &        $0.00235$   \\
         TopHAT & $I$ & $2453875.95723$   &     $0.98086$   &        $0.00257$   \\
         TopHAT & $I$ & $2453875.95981$   &     $0.98294$   &        $0.00257$   \\
         TopHAT & $I$ & $2453875.96237$   &     $0.98489$   &        $0.00216$   \\
         TopHAT & $I$ & $2453875.96495$   &     $0.99114$   &        $0.00289$   \\
         TopHAT & $I$ & $2453875.96752$   &     $0.98283$   &        $0.00216$   \\
         TopHAT & $I$ & $2453875.97010$   &     $0.98710$   &        $0.00244$   \\
         TopHAT & $I$ & $2453875.97268$   &     $0.98623$   &        $0.00235$   \\
         TopHAT & $I$ & $2453875.97523$   &     $0.99019$   &        $0.00239$   \\
         TopHAT & $I$ & $2453875.97778$   &     $0.99540$   &        $0.00266$   \\
         TopHAT & $I$ & $2453875.98031$   &     $0.99495$   &        $0.00299$   \\
         TopHAT & $I$ & $2453879.63599$   &     $0.99150$   &        $0.00794$   \\
         TopHAT & $I$ & $2453879.63854$   &     $1.00323$   &        $0.00677$   \\
         TopHAT & $I$ & $2453879.64108$   &     $0.99596$   &        $0.00488$   \\
         TopHAT & $I$ & $2453879.64361$   &     $0.99935$   &        $0.00404$   \\
         TopHAT & $I$ & $2453879.64620$   &     $1.00261$   &        $0.00384$   \\
         TopHAT & $I$ & $2453879.64874$   &     $1.00076$   &        $0.00410$   \\
         TopHAT & $I$ & $2453879.65128$   &     $1.00229$   &        $0.00469$   \\
         TopHAT & $I$ & $2453879.65382$   &     $0.99927$   &        $0.00436$   \\
         TopHAT & $I$ & $2453879.66923$   &     $0.99853$   &        $0.00371$   \\
         TopHAT & $I$ & $2453879.67945$   &     $0.99478$   &        $0.00345$   \\
         TopHAT & $I$ & $2453879.68494$   &     $1.00971$   &        $0.00384$   \\
         TopHAT & $I$ & $2453879.69258$   &     $1.00096$   &        $0.00404$   \\
         TopHAT & $I$ & $2453879.70278$   &     $1.00239$   &        $0.00319$   \\
         TopHAT & $I$ & $2453879.70533$   &     $0.99817$   &        $0.00371$   \\
         TopHAT & $I$ & $2453879.71041$   &     $1.00221$   &        $0.00351$   \\
         TopHAT & $I$ & $2453879.71554$   &     $0.99585$   &        $0.00293$   \\
         TopHAT & $I$ & $2453879.71808$   &     $0.99825$   &        $0.00371$   \\
         TopHAT & $I$ & $2453879.72061$   &     $0.99912$   &        $0.00339$   \\
         TopHAT & $I$ & $2453879.72570$   &     $1.00209$   &        $0.00312$   \\
         TopHAT & $I$ & $2453879.73078$   &     $1.00025$   &        $0.00306$   \\
         TopHAT & $I$ & $2453879.73374$   &     $0.99631$   &        $0.00312$   \\
         TopHAT & $I$ & $2453879.73627$   &     $0.99526$   &        $0.00358$   \\
         TopHAT & $I$ & $2453879.74390$   &     $0.99428$   &        $0.00325$   \\
         TopHAT & $I$ & $2453879.74645$   &     $1.00067$   &        $0.00319$   \\
         TopHAT & $I$ & $2453879.74899$   &     $0.99849$   &        $0.00267$   \\
         TopHAT & $I$ & $2453879.75409$   &     $0.99504$   &        $0.00267$   \\
         TopHAT & $I$ & $2453879.76425$   &     $0.99602$   &        $0.00319$   \\
         TopHAT & $I$ & $2453879.76679$   &     $0.99473$   &        $0.00293$   \\
         TopHAT & $I$ & $2453879.76933$   &     $0.99675$   &        $0.00312$   \\
         TopHAT & $I$ & $2453879.77188$   &     $0.99841$   &        $0.00365$   \\
         TopHAT & $I$ & $2453879.77442$   &     $0.99830$   &        $0.00319$   \\
         TopHAT & $I$ & $2453879.77695$   &     $0.99937$   &        $0.00260$   \\
         TopHAT & $I$ & $2453879.78204$   &     $0.99869$   &        $0.00280$   \\
         TopHAT & $I$ & $2453879.78500$   &     $0.99970$   &        $0.00267$   \\
         TopHAT & $I$ & $2453879.78755$   &     $0.99944$   &        $0.00306$   \\
         TopHAT & $I$ & $2453879.79010$   &     $1.00770$   &        $0.00319$   \\
         TopHAT & $I$ & $2453879.79270$   &     $1.00215$   &        $0.00325$   \\
         TopHAT & $I$ & $2453879.79524$   &     $1.00284$   &        $0.00332$   \\
         TopHAT & $I$ & $2453879.79778$   &     $1.00141$   &        $0.00371$   \\
         TopHAT & $I$ & $2453879.80286$   &     $1.00342$   &        $0.00345$   \\
         TopHAT & $I$ & $2453879.80796$   &     $0.99913$   &        $0.00260$   \\
         TopHAT & $I$ & $2453879.81049$   &     $0.99415$   &        $0.00436$   \\
         TopHAT & $I$ & $2453879.81303$   &     $0.99213$   &        $0.00345$   \\
         TopHAT & $I$ & $2453879.82066$   &     $0.98650$   &        $0.00274$   \\
         TopHAT & $I$ & $2453879.82573$   &     $0.98379$   &        $0.00293$   \\
         TopHAT & $I$ & $2453879.82827$   &     $0.98645$   &        $0.00286$   \\
         TopHAT & $I$ & $2453879.83081$   &     $0.98465$   &        $0.00274$   \\
         TopHAT & $I$ & $2453879.83335$   &     $0.98752$   &        $0.00235$   \\
         TopHAT & $I$ & $2453879.83632$   &     $0.98410$   &        $0.00293$   \\
         TopHAT & $I$ & $2453879.83886$   &     $0.98172$   &        $0.00280$   \\
         TopHAT & $I$ & $2453879.84140$   &     $0.98134$   &        $0.00286$   \\
         TopHAT & $I$ & $2453879.84648$   &     $0.97897$   &        $0.00280$   \\
         TopHAT & $I$ & $2453879.84908$   &     $0.98167$   &        $0.00306$   \\
         TopHAT & $I$ & $2453879.85164$   &     $0.98046$   &        $0.00247$   \\
         TopHAT & $I$ & $2453879.85418$   &     $0.98182$   &        $0.00260$   \\
         TopHAT & $I$ & $2453879.85672$   &     $0.98162$   &        $0.00241$   \\
         TopHAT & $I$ & $2453879.86181$   &     $0.98019$   &        $0.00267$   \\
         TopHAT & $I$ & $2453879.86434$   &     $0.98286$   &        $0.00286$   \\
         TopHAT & $I$ & $2453879.86689$   &     $0.98298$   &        $0.00286$   \\
         TopHAT & $I$ & $2453879.86942$   &     $0.98211$   &        $0.00280$   \\
         TopHAT & $I$ & $2453879.87196$   &     $0.98143$   &        $0.00274$   \\
         TopHAT & $I$ & $2453879.87450$   &     $0.98296$   &        $0.00293$   \\
         TopHAT & $I$ & $2453879.87704$   &     $0.97995$   &        $0.00254$   \\
         TopHAT & $I$ & $2453879.87958$   &     $0.97947$   &        $0.00280$   \\
         TopHAT & $I$ & $2453879.88213$   &     $0.98161$   &        $0.00247$   \\
         TopHAT & $I$ & $2453879.88467$   &     $0.98646$   &        $0.00339$   \\
         TopHAT & $I$ & $2453879.88764$   &     $0.97974$   &        $0.00300$   \\
         TopHAT & $I$ & $2453879.89017$   &     $0.98523$   &        $0.00286$   \\
         TopHAT & $I$ & $2453879.89271$   &     $0.98085$   &        $0.00274$   \\
         TopHAT & $I$ & $2453879.89525$   &     $0.98558$   &        $0.00312$   \\
         TopHAT & $I$ & $2453879.89778$   &     $0.98520$   &        $0.00306$   \\
         TopHAT & $I$ & $2453879.90033$   &     $0.98688$   &        $0.00254$   \\
         TopHAT & $I$ & $2453879.90287$   &     $0.98446$   &        $0.00325$   \\
         TopHAT & $I$ & $2453879.90542$   &     $0.98404$   &        $0.00306$   \\
         TopHAT & $I$ & $2453879.90796$   &     $0.98488$   &        $0.00325$   \\
         TopHAT & $I$ & $2453879.91049$   &     $0.98793$   &        $0.00267$   \\
         TopHAT & $I$ & $2453879.91304$   &     $0.98835$   &        $0.00286$   \\
         TopHAT & $I$ & $2453879.91557$   &     $0.99358$   &        $0.00286$   \\
         TopHAT & $I$ & $2453879.91812$   &     $0.99742$   &        $0.00293$   \\
         TopHAT & $I$ & $2453879.92067$   &     $0.99568$   &        $0.00260$   \\
         TopHAT & $I$ & $2453879.92320$   &     $0.99590$   &        $0.00286$   \\
         TopHAT & $I$ & $2453879.92575$   &     $0.99512$   &        $0.00286$   \\
         TopHAT & $I$ & $2453879.92829$   &     $0.99686$   &        $0.00319$   \\
         TopHAT & $I$ & $2453879.93083$   &     $1.00214$   &        $0.00384$   \\
         TopHAT & $I$ & $2453879.93338$   &     $0.99751$   &        $0.00286$   \\
         TopHAT & $I$ & $2453879.93593$   &     $0.99948$   &        $0.00345$   \\
         TopHAT & $I$ & $2453879.93889$   &     $1.00122$   &        $0.00254$   \\
         TopHAT & $I$ & $2453879.94143$   &     $1.00059$   &        $0.00306$   \\
         TopHAT & $I$ & $2453879.94397$   &     $0.99564$   &        $0.00286$   \\
         TopHAT & $I$ & $2453879.94652$   &     $1.00071$   &        $0.00332$   \\
         TopHAT & $I$ & $2453879.94905$   &     $0.99877$   &        $0.00260$   \\
         TopHAT & $I$ & $2453879.95159$   &     $1.00199$   &        $0.00300$   \\
         TopHAT & $I$ & $2453879.95413$   &     $0.99867$   &        $0.00293$   \\
         TopHAT & $I$ & $2453879.95668$   &     $1.00033$   &        $0.00267$   \\
         TopHAT & $I$ & $2453879.95922$   &     $1.00162$   &        $0.00306$   \\
         TopHAT & $I$ & $2453879.96176$   &     $0.99868$   &        $0.00325$   \\
         TopHAT & $I$ & $2453879.96430$   &     $1.00137$   &        $0.00306$   \\
         TopHAT & $I$ & $2453879.96688$   &     $0.99675$   &        $0.00300$   \\
         TopHAT & $I$ & $2453879.96945$   &     $0.99985$   &        $0.00345$   \\
         TopHAT & $I$ & $2453879.97202$   &     $0.99857$   &        $0.00319$   \\
         TopHAT & $I$ & $2453883.64043$   &     $0.99501$   &        $0.00401$   \\
         TopHAT & $I$ & $2453883.64551$   &     $1.00869$   &        $0.00374$   \\
         TopHAT & $I$ & $2453883.65317$   &     $1.00715$   &        $0.00363$   \\
         TopHAT & $I$ & $2453883.65824$   &     $1.00015$   &        $0.00384$   \\
         TopHAT & $I$ & $2453883.66597$   &     $1.00241$   &        $0.00395$   \\
         TopHAT & $I$ & $2453883.66850$   &     $0.99770$   &        $0.00294$   \\
         TopHAT & $I$ & $2453883.67359$   &     $1.00034$   &        $0.00379$   \\
         TopHAT & $I$ & $2453883.68119$   &     $0.99916$   &        $0.00384$   \\
         TopHAT & $I$ & $2453883.69436$   &     $0.99367$   &        $0.00326$   \\
         TopHAT & $I$ & $2453883.69949$   &     $1.00261$   &        $0.00321$   \\
         TopHAT & $I$ & $2453883.71996$   &     $1.00687$   &        $0.00321$   \\
         TopHAT & $I$ & $2453883.72764$   &     $0.99723$   &        $0.00310$   \\
         TopHAT & $I$ & $2453883.73016$   &     $0.99798$   &        $0.00310$   \\
         TopHAT & $I$ & $2453883.73820$   &     $0.99884$   &        $0.00331$   \\
         TopHAT & $I$ & $2453883.74328$   &     $0.99660$   &        $0.00315$   \\
         TopHAT & $I$ & $2453883.74835$   &     $0.99696$   &        $0.00283$   \\
         TopHAT & $I$ & $2453883.75090$   &     $0.98876$   &        $0.00299$   \\
         TopHAT & $I$ & $2453883.75343$   &     $0.99050$   &        $0.00304$   \\
         TopHAT & $I$ & $2453883.76105$   &     $0.97861$   &        $0.00288$   \\
         TopHAT & $I$ & $2453883.76613$   &     $0.98150$   &        $0.00310$   \\
         TopHAT & $I$ & $2453883.76866$   &     $0.98266$   &        $0.00283$   \\
         TopHAT & $I$ & $2453883.77121$   &     $0.97916$   &        $0.00246$   \\
         TopHAT & $I$ & $2453883.77374$   &     $0.98116$   &        $0.00261$   \\
         TopHAT & $I$ & $2453883.77881$   &     $0.98531$   &        $0.00251$   \\
         TopHAT & $I$ & $2453883.79199$   &     $0.98102$   &        $0.00251$   \\
         TopHAT & $I$ & $2453883.80221$   &     $0.98419$   &        $0.00288$   \\
         TopHAT & $I$ & $2453883.80474$   &     $0.98467$   &        $0.00267$   \\
         TopHAT & $I$ & $2453883.81497$   &     $0.98451$   &        $0.00304$   \\
         TopHAT & $I$ & $2453883.82003$   &     $0.97703$   &        $0.00267$   \\
         TopHAT & $I$ & $2453883.82766$   &     $0.98075$   &        $0.00267$   \\
         TopHAT & $I$ & $2453883.83020$   &     $0.98536$   &        $0.00294$   \\
         TopHAT & $I$ & $2453883.83274$   &     $0.98276$   &        $0.00310$   \\
         TopHAT & $I$ & $2453883.84078$   &     $0.98421$   &        $0.00246$   \\
         TopHAT & $I$ & $2453883.85602$   &     $0.98902$   &        $0.00241$   \\
         TopHAT & $I$ & $2453883.86110$   &     $0.99461$   &        $0.00310$   \\
         TopHAT & $I$ & $2453883.86873$   &     $0.99717$   &        $0.00310$   \\
         TopHAT & $I$ & $2453883.87128$   &     $1.00104$   &        $0.00304$   \\
         TopHAT & $I$ & $2453883.87382$   &     $1.00207$   &        $0.00331$   \\
         TopHAT & $I$ & $2453883.87890$   &     $0.99948$   &        $0.00288$   \\
         TopHAT & $I$ & $2453883.88398$   &     $1.00209$   &        $0.00299$   \\
         TopHAT & $I$ & $2453883.88652$   &     $1.00186$   &        $0.00294$   \\
         TopHAT & $I$ & $2453883.89201$   &     $0.99835$   &        $0.00304$   \\
         TopHAT & $I$ & $2453883.89965$   &     $0.99958$   &        $0.00267$   \\
         TopHAT & $I$ & $2453883.90472$   &     $0.99636$   &        $0.00321$   \\
         TopHAT & $I$ & $2453883.90980$   &     $0.99640$   &        $0.00283$   \\
         TopHAT & $I$ & $2453883.91489$   &     $0.99838$   &        $0.00278$   \\
         TopHAT & $I$ & $2453883.91743$   &     $0.99901$   &        $0.00288$   \\
         TopHAT & $I$ & $2453883.92505$   &     $0.99920$   &        $0.00321$   \\
         TopHAT & $I$ & $2453883.92758$   &     $1.00209$   &        $0.00304$   \\
         TopHAT & $I$ & $2453883.93012$   &     $0.99552$   &        $0.00321$   \\
         TopHAT & $I$ & $2453883.93269$   &     $1.00333$   &        $0.00347$   \\
         TopHAT & $I$ & $2453883.93528$   &     $1.00105$   &        $0.00294$   \\
         TopHAT & $I$ & $2453883.93787$   &     $1.00112$   &        $0.00315$   \\
         TopHAT & $I$ & $2453883.94091$   &     $0.99854$   &        $0.00326$   \\
         TopHAT & $I$ & $2453883.94350$   &     $0.99875$   &        $0.00304$   \\
         TopHAT & $I$ & $2453883.94609$   &     $1.00058$   &        $0.00310$   \\
         TopHAT & $I$ & $2453883.94868$   &     $0.99873$   &        $0.00251$   \\
         TopHAT & $I$ & $2453883.95128$   &     $0.99768$   &        $0.00342$   \\
         TopHAT & $I$ & $2453883.95385$   &     $1.00243$   &        $0.00294$   \\
         TopHAT & $I$ & $2453883.95892$   &     $0.99752$   &        $0.00288$   \\
         TopHAT & $I$ & $2453883.96146$   &     $0.99345$   &        $0.00369$   \\
         TopHAT & $I$ & $2453883.96401$   &     $0.99281$   &        $0.00342$   \\
         TopHAT & $I$ & $2453883.96658$   &     $0.99945$   &        $0.00342$   \\
         TopHAT & $I$ & $2453883.96920$   &     $0.99881$   &        $0.00342$   \\
         TopHAT & $I$ & $2453883.97175$   &     $1.00105$   &        $0.00352$   \\
         TopHAT & $I$ & $2453883.97430$   &     $1.00180$   &        $0.00347$   \\
         TopHAT & $I$ & $2453883.97684$   &     $1.00327$   &        $0.00363$   \\
\enddata 

\tablecomments{The time stamps represent the Heliocentric Julian Date
  at the time of mid-exposure. The uncertainty estimates are based on
  the procedures described in \S~2. We intend for this Table to appear
  in entirety in the electronic version of the journal. A portion is
  shown here to illustrate its format. The data are also available in
  digital from the authors upon request.}

\end{deluxetable}

